CRANE: Reasoning with constrained LLM generation

Code generation, symbolic math reasoning, and other tasks require LLMs to produce outputs that are both syntactically and semantically correct. Constrained LLM generation is a promising direction to enforce adherence to formal grammar, but prior works have empirically observed that strict enforcement of formal constraints often diminishes the reasoning capabilities of LLMs. In this work, we first provide a theoretical explanation for why constraining LLM outputs to very restrictive grammars that only allow syntactically valid final answers reduces the reasoning capabilities of the model. Second, we demonstrate that by augmenting the output grammar with carefully designed additional rules, it is always possible to preserve the reasoning capabilities of the LLM while ensuring syntactic and semantic correctness in its outputs. Building on these theoretical insights, we propose a reasoning-augmented constrained decoding algorithm, CRANE, which effectively balances the correctness of constrained generation with the flexibility of unconstrained generation. Experiments on multiple open-source LLMs and benchmarks show that CRANE significantly outperforms both state-of-the-art constrained decoding strategies and standard unconstrained decoding, showing up to 10% points accuracy improvement over baselines on challenging symbolic reasoning benchmarks GSM-symbolic and FOLIO.

==> algorithms/crane.tex <==
% \begin{algorithm}
% \small
% \caption{LLM Generation with \Tool{}}
% \label{alg:crane}
% \begin{flushleft}
% \textbf{Inputs:} 
% \begin{itemize}
%     \item LLM: A language model capable of generating token scores.
%     \item curr\_tokens: The current sequence of tokens.
%     \item tokenizer: A tokenizer for encoding and decoding tokens.
%     \item constraint\_tool: A tool for enforcing grammatical constraints.
%     \item output\_grammar: The grammar to be enforced during generation.
%     \item start\_symbol: The symbol indicating the start of a constrained generation.
%     \item end\_symbol: The symbol indicating the end of a constrained generation.
% \end{itemize}

% \textbf{Output:} A generated sequence of tokens adhering to the specified grammar.

% \begin{algorithmic}[1]
% \Function{crane}{LLM, curr\_tokens, tokenizer, constraint\_tool, output\_grammar, start\_symbol, end\_symbol}
% \State $\text{output\_grammar} \gets \text{add\_special\_symbols}(\text{output\_grammar}, \text{start\_symbol}, \text{end\_symbol})$
% \State $\text{constraint\_tool.initialize}(\text{output\_grammar})$
% \State $\text{overall\_gen} \gets \text{''}$
% \State $\text{structured\_gen} \gets \text{''}$
% \State $\text{current\_state} \gets \text{Unconstrained}$
% \State $\text{last\_constrained\_end} \gets \text{len}(\text{curr\_tokens}) - 1$

% \While{True}
%     \If{$\text{current\_state} == \text{Constrained}$ \textbf{and} $\text{structured\_gen.endswith}(\text{end\_symbol})$}
%         \State $\text{constraint\_tool.parser.reset}()$
%         \State $\text{current\_state} \gets \text{Unconstrained}$
%         \State $\text{last\_constrained\_end} \gets \text{len}(\text{curr\_tokens}) - 1$
%     \EndIf

%     \State $\text{scores} \gets \text{LLM}(\text{curr\_tokens})$

%     \If{$\text{current\_state} == \text{Constrained}$}
%         \State $\text{structured\_gen} \gets \text{detokenize}(\text{tokenizer}, \text{curr\_tokens}[:, \text{start\_constrained\_from}:])$
%         \State $\text{constraint\_tool.parser.update}(\text{start\_symbol} + \text{structured\_gen})$
%         \State $\text{m} \gets \text{generate\_mask}(\text{constraint\_tool.parser})$
%         \State $\text{scores} \gets \text{m} \odot \text{scores}$
%     \EndIf

%     \State $\text{t\_i} \gets \text{decoding\_algorithm}(\text{scores})$

%     \If{$\text{t\_i} == \text{EOS}$}
%         \State \textbf{break}
%     \EndIf

%     \State $\text{curr\_tokens} \gets \text{append}(\text{curr\_tokens}, \text{t\_i})$

%     \If{$\text{current\_state} == \text{Unconstrained}$}
%         \State $\text{unstructured\_gen} \gets \text{detokenize}(\text{tokenizer}, \text{curr\_tokens}[:, \text{last\_constrained\_end} + 1:])$
%         \If{$\text{start\_symbol} \in \text{unstructured\_gen}$}
%             \State $\text{start\_constrained\_from} \gets \text{len}(\text{curr\_tokens})$
%             \State $\text{current\_state} \gets \text{Constrained}$
%         \EndIf
%     \EndIf

%     \State $\text{overall\_gen} \gets \text{detokenize}(\text{tokenizer}, \text{curr\_tokens})$

%     \If{$\text{len}(\text{curr\_tokens}) > \text{max\_tokens}$}
%         \State \textbf{break}
%     \EndIf
% \EndWhile

% \State \textbf{return} $\text{overall\_gen}$
% \EndFunction
% \end{algorithmic}
% \end{flushleft}
% \end{algorithm}
